Reward-Free Curricula for Training Robust World Models

There has been a recent surge of interest in developing generally-capable agents that can adapt to new tasks without additional training in the environment. Learning world models from reward-free exploration is a promising approach, and enables policies to be trained using imagined experience for new tasks. However, achieving a general agent requires robustness across different environments. In this work, we address the novel problem of generating curricula in the reward-free setting to train robust world models. We consider robustness in terms of minimax regret over all environment instantiations and show that the minimax regret can be connected to minimising the maximum error in the world model across environment instances. This result informs our algorithm, WAKER: Weighted Acquisition of Knowledge across Environments for Robustness. WAKER selects environments for data collection based on the estimated error of the world model for each environment. Our experiments demonstrate that WAKER outperforms several baselines, resulting in improved robustness, efficiency, and generalisation.

==> tex/acknowledgements.tex <==
%!TEX root = ../iclr2024_conference.tex
\section*{Acknowledgements}

This work was supported by a Programme Grant from the Engineering and Physical Sciences Research
Council (EP/V000748/1) and a gift from Amazon
Web Services. Additionally, this project made use of the Tier 2 HPC facility JADE2, funded by
the Engineering and Physical Sciences Research Council (EP/T022205/1).

==> tex/algos/waker0.tex <==
\algtext*{EndWhile}
\algtext*{EndFor}
\algtext*{EndIf}
\algtext*{EndProcedure}
\algtext*{EndFunction}

% \begin{wrapfigure}{r}{0.5\linewidth}
\begin{minipage}[!b]{\linewidth}
\begin{algorithm}
    \small
    \caption{Weighted Acquisition of Knowledge across Environments for Robustness (WAKER)}\label{alg:WAKER}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        \State \textbf{Require:}   UPOMDP with free parameters $\Theta$; Boltzmann temperature $\textnormal{\texttt{T}}_{\textnormal{\texttt{B}}}$; Imagination horizon $h$;

        \State \textbf{Initialise:} Data Buffer, $D$; Error Estimate Buffer, $D_{\textnormal{error}}$; World Model $W = \{q, \widehat{T}\}$; Exploration Policy $\pi^{\textnormal{expl}}$; \vspace{2.5mm}
         
        \While{\textnormal{training world model}} 
        \If{$p \sim U_{[0, 1]} < p_{\textnormal{DR}}$ or $D$.\texttt{is\_empty}()}
            \State $\theta \sim$ \texttt{DomainRandomisation}$(\Theta)$ \label{algline:dr}
        \Else
        \State $\theta \sim$ \texttt{Boltzmann}(\texttt{Normalize}($ D_{\textnormal{error}}), \textnormal{\texttt{T}}_{\textnormal{\texttt{B}}})$ \label{algline:boltzmann}
        \EndIf
        \State $\tau_\theta$ $\leftarrow $ rollout of $\pi^{\textnormal{expl}}$ in $\mathcal{P}_\theta$ \Comment{Collect real trajectory in environment with parameter $\theta$} \label{algline:real_rollout}
        \State $D$.\texttt{add}(\{$\tau_\theta$\}) \Comment{Add trajectory to $D$ labelled with $\theta$}
        \State train $W$ on $D$ \label{algline:train_wm}
        \State $\pi^{\textnormal{expl}}$, $D_{\textnormal{error}} \leftarrow$ \texttt{Imagine}($D$, $D_{\textnormal{error}}$, $W$, $\pi^{\textnormal{expl}}$)  \Comment{Perform rollouts in imagination} \label{algline:call_imagine} \vspace{2.5mm}
        \EndWhile
        \Function{\textnormal{\texttt{Imagine}}}{$D$, $D_{\textnormal{error}}$, $W$, $\pi^{\textnormal{expl}}$} 
            \For{$i = 1, \dots, K$} \Comment{Batch of imagination rollouts}
                \State $\tau_\theta \leftarrow D$.\texttt{sample}() \Comment{Sample trajectory from data buffer} \label{algline:sample_ep}
                \State $Z_{{\tau_\theta}} = \{z_t\}_{t=0}^{|\tau_\theta|}\leftarrow q($e$_\theta$)  \Comment{Encode trajectory into latent states} \label{algline:encode}
                \State $\widehat{\textnormal{e}}_\theta$ $\leftarrow $ rollout $\pi^{\textnormal{expl}}$ for $h$ steps starting from $z \in Z_{{\tau_\theta}}$ using $\widehat{T}$ \Comment{Imagination rollout} \label{algline:imagine}
                \State error\_estimate $\leftarrow  \frac{1}{h} \sum_{z, a \in \widehat{\textnormal{e}}_\theta} \big[\textnormal{Var}\big\{\mathbb{E}[ \widehat{T}_i( \cdot | z, a) ]\big\}_{i=1}^N \big] $ \Comment{Evaluate Equation~\ref{eq:wm_error_approx} on $\widehat{\textnormal{e}}_\theta$} \label{algline:error_est}
                \State \texttt{update}($D_{\textnormal{error}}$, error\_estimate, $\theta$)\Comment{Update error estimate for $\theta$} \label{algline:error_update}
                \State train $\pi^{\textnormal{expl}}$ on $\widehat{\tau_\theta}$ \label{algline:train_expl}
            \EndFor
            \Return $\pi^{\textnormal{expl}}$, $D_{\textnormal{error}}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}
\end{minipage}
% \end{wrapfigure}

